Equivariance versus Augmentation for Spherical Images

We analyze the role of rotational equivariance in convolutional neural networks (CNNs) applied to spherical images. We compare the performance of the group equivariant networks known as S2CNNs and standard non-equivariant CNNs trained with an increasing amount of data augmentation. The chosen architectures can be considered baseline references for the respective design paradigms. Our models are trained and evaluated on single or multiple items from the MNIST or FashionMNIST dataset projected onto the sphere. For the task of image classification, which is inherently rotationally invariant, we find that by considerably increasing the amount of data augmentation and the size of the networks, it is possible for the standard CNNs to reach at least the same performance as the equivariant network. In contrast, for the inherently equivariant task of semantic segmentation, the non-equivariant networks are consistently outperformed by the equivariant networks with significantly fewer parameters. We also analyze and compare the inference latency and training times of the different networks, enabling detailed tradeoff considerations between equivariant architectures and data augmentation for practical problems. The equivariant spherical networks used in the experiments are available at https://github.com/JanEGerken/sem_seg_s2cnn .

==> section_spherical_convolutions.tex <==
\section{Spherical convolutions}
\label{sec:spherical}
\noindent In this section, we will investigate the spherical convolutions introduced in Example~\ref{ex:sphericalCNN} in more detail. Mathematically, this case is particularly interesting, because on the sphere and on $\SO(3)$, we can leverage the power of the rich spectral theory on the sphere in terms of spherical harmonics and Wigner matrices to find explicit and compact expressions for the convolutions. Also for practical considerations, this case is of particular importance since data given on a sphere arises naturally in many applications, e.g.\ for fisheye cameras~\cite{coors2018}, cosmological data~\cite{perraudin2019}, weather data, molecular modeling~\cite{boomsma2017} or diffusion MRI~\cite{elaldi2021}. To faithfully represent this data, equivariant convolutions are essential.

There is a sizable literature on equivariant spherical convolutions. The approach presented here follows \cite{cohen2018b} and extends the results in the reference at some points. An overview of the existing literature in the field can be found in Section~\ref{sec:related-literature}.

\subsection{Preliminaries}
For spherical CNNs, the input data has the form $f:S^{2}\rightarrow \RR^{\Nc}$, i.e. the first layer of the network has $\mathcal{X}=S^{2}$. The networks discussed here are special cases of the GCNNs constructed in Section~\ref{sec:equiv-conv-layers} for which the symmetry group $G$ is the rotation group in three dimensions, $\SO(3)$ and the subgroup $K$ is either $\SO(2)$ or trivial. In this framework, we identify $S^{2}$ with the homogeneous space $G/K=\SO(3)/\SO(2)$. The first layer of the network has trivial $K$ in the output, i.e. \ $\mathcal{Y}=\SO(3)$ and subsequent layers have trivial $K$ also in the input, i.e.\ $\mathcal{X}=\mathcal{Y}=\SO(3)$. The latter case was already discussed in Example~\ref{ex:sphericalCNN}, leading to~\eqref{SO3C_conv}.

For the first layer, $\SO(3)$ acts by the matrix-vector product on the input space, $\sigma_{1}(R)x=Rx$ and as usual by group multiplication on the output, $\sigma_{2}(R)Q=RQ$. The construction in \cite{cohen2018b} uses in this case the identity element in $\mathcal{Y}=\SO(3)$ to solve the kernel constraint, leading to
\begin{align}
  (\kappa \star f)(R) = \int_{S^{2}}\rho_{2}(R)\kappa(R^{-1}x)\rho_{1}^{-1}(R)f(x)\,\dd{x}\,,\label{eq:28}
\end{align}
cf.\ \eqref{eq:1}. The integration measure on the sphere is given by
\begin{align}
  \int_{S^{2}}\dd{x(\theta,\varphi)}=\int_{0}^{2\pi}\dd{\varphi}\int_{0}^{\pi}\dd{\theta}\sin\theta\,.
\end{align}
Note that in~\eqref{eq:28} we perform the integral here over the input domain $\mathcal{X}$ and not the symmetry group $G$ since we cannot replace the integral over $\mathcal{X}$ by an integral over $G$ if we use a reference point in $\mathcal{Y}$, as mentioned above.

\begin{remark}[Convolutions with $\mathcal{X}=\mathcal{Y}=S^{2}$]
\label{rk:isotropic}
  At first, it might seem counter-intuitive that the feature maps in a spherical CNN have domain $\SO(3)$ instead of $S^{2}$ after the first layer. Hence, it is instructive to study a convolutional integral with $\mathcal{X}=\mathcal{Y}=S^{2}$ constructed using the techniques of Section~\ref{sec:GC}. The action of $\SO(3)$ on $S^{2}$ is as above by matrix-vector product. We next choose an arbitrary reference point $x_{0}$ on the sphere and denote by $R_{x}$ the rotation matrix which rotates $x_{0}$ into $x$: $R_{x}x_{0}=x$. Following~\eqref{GC_conv}, we can then write the convolution as
  \begin{align}
    [\kappa\star f](y)=\int_{\mathcal{X}}\rho_{2}(R_{x})\kappa(R_{x}^{-1}y)\rho_{1}^{-1}(R_{x})f(x)\,\dd{x}\,.\label{eq:7}
  \end{align}
  However, the element $R_{x}$ is not unique: If $Q$ rotates around $x_{0}$, $Qx_{0}=x_{0}$, then $R_{x}Q$ also rotates $x_{0}$ into $x$. In fact, the symmetry group splits into a semi-direct product $\SO(3)=N\rtimes H$ with $H=\SO(2)$ the stabilizer of $x_{0}$ and $N=\SO(3)/H$. This special case was considered in Section~\ref{sec:sem_dir_prod_grps} and we can write~\eqref{eq:7} as
  \begin{align}
    [\kappa\star f](y)=\int_{\SO(3)/H}\rho_{2}(R)\kappa(R^{-1}y)\rho_{1}^{-1}(R)f(R x_{0})\,\dd{R}\,.
  \end{align}
  According to~\eqref{eq:23}, the kernel $\kappa$ is now not unconstrained anymore but satisfies
  \begin{align}
    \kappa(Qy)=\rho_{2}(Q)\kappa(y)\rho_{1}^{-1}(Q)\,,\label{eq:25}
  \end{align}
  for $Q\in H$. In particular, if the input and output features transform like scalars, $\rho_{1}=\rho_{2}=\id$, \eqref{eq:25} implies that the kernel is invariant under rotations around $x_{0}$, i.e.\ isotropic, as was noticed also in \cite{makadia2007}. In practice, this isotropy decreases the expressibility of the layer considerably.
\end{remark}

\subsection{Spherical convolutions and Fourier transforms}
\label{sec:spherFourier}
The Fourier decomposition on the sphere and on $\SO(3)$ is well studied and can be used to find compact explicit expressions for the integrals defined in the previous section. To simplify some expressions, we will assume in this and the following section that $V_{1,2}$ are vector spaces over $\RR$, so in particular $\rho_{1,2}$ are real representations.

A square-integrable function $f:S^{2}\rightarrow \RR^{c}$ can be decomposed into the spherical harmonics $Y^{\ell}_{m}$ via
\begin{align}
  f(x)=\sum_{\ell=0}^{\infty}\sum_{m=-\ell}^{\ell} \hat{f}_{m}^{\ell}Y^{\ell}_{m}(x)\,,
\end{align}
with Fourier coefficients
\begin{align}
  \hat{f}^{\ell}_{m}=\int_{S^{2}}f(x) \overline{Y^{\ell}_{m}(x)}\ \dd{x}\,,
\end{align}
since the spherical harmonics form a complete orthogonal set,
\begin{align}
  \sum_{\ell=0}^{\infty}\sum_{m=-\ell}^{\ell}\overline{Y^{\ell}_{m}(x)}Y^{\ell}_{m}(y)&=\delta(x-y)\,,\\
  \int_{S^{2}}\overline{Y^{\ell_{1}}_{m_{1}}(x)}Y^{\ell_{2}}_{m_{2}}(x)\dd{x}&=\delta_{\ell_{1}\ell_{2}}\delta_{m_{1}m_{2}}\,.
\end{align}
For later convenience, we also note the following property of spherical harmonics:
\begin{align}
  \overline{Y^{\ell}_{m}(x)}=(-1)^{\ell}Y^{\ell}_{-m}(x)\,.\label{eq:16}
\end{align}
In practice, one truncates the sum over $\ell$ at some finite $L$, the bandwidth, obtaining an approximation of $f$.

Similarly, a square-integrable function $f:\SO(3)\rightarrow \RR^{c}$ can be decomposed into Wigner D-matrices $\mathcal{D}^{\ell}_{mn}(R)$ (for a comprehensive review, see \cite{varshalovich1988}) via
\begin{align}
  f(R)=\sum_{\ell=0}^{\infty}\sum_{m,n=-\ell}^{\ell}\hat{f}^{\ell}_{mn}\mathcal{D}^{\ell}_{mn}(R)\,,\label{eq:26}
\end{align}
with Fourier coefficients
\begin{align}
  \hat{f}^{\ell}_{mn}=\frac{2\ell+1}{8\pi^{2}}\int_{\SO(3)}f(R) \overline{\mathcal{D}^{\ell}_{mn}(R)}\ \dd{R}\,,\label{eq:27}
\end{align}
since the Wigner matrices satisfy the orthogonality and completeness relations
\begin{align}
  \int_{\SO(3)}\overline{\mathcal{D}^{\ell_{1}}_{m_{1}n_{1}}(R)}\mathcal{D}^{\ell_{2}}_{m_{2}n_{2}}(R)\dd{R}&=\frac{8\pi^{2}}{2\ell_{1}+1}\delta_{\ell_{1}\ell_{2}}\delta_{m_{1}m_{2}}\delta_{n_{1}n_{2}}\,\\
  \sum_{\ell=0}^{\infty}\sum_{m,n=-\ell}^{\ell}\overline{\mathcal{D}^{\ell}_{mn}(Q)}\mathcal{D}^{\ell}_{mn}(R)&=\frac{8\pi^{2}}{2\ell+1}\delta(R-Q)\,.
\end{align}
Furthermore, the Wigner D-matrices form a unitary representation of $\SO(3)$ since they satisfy
\begin{align}  
  \mathcal{D}^{\ell}_{mn}(QR) &= \sum_{p=-\ell}^{\ell} \mathcal{D}^{\ell}_{mp}(Q) \mathcal{D}^{\ell}_{pn}(R)\,,\\
  \mathcal{D}^{\ell}_{mn}(R^{-1}) &= (\mathcal{D}^{\ell}_{mn}(R))^{-1}=(\mathcal{D}^{\ell}_{mn}(R))^{\dagger} = \overline{\mathcal{D}^{\ell}_{nm}(R)} \,.
\end{align}
Note furthermore that
\begin{align}
  \overline{\mathcal{D}^{\ell}_{mn}(R)}=(-1)^{n-m}\mathcal{D}^{\ell}_{-m,-n}(R)\,.\label{eq:13}
\end{align}
The regular representation of $\SO(3)$ on spherical harmonics of order $\ell$ is given by the corresponding Wigner matrices:
\begin{align}
  Y^{\ell}_{m}(Rx)=\sum_{n=-\ell}^{\ell}\overline{\mathcal{D}^{\ell}_{mn}(R)}Y^{\ell}_{n}(x)\,.\label{eq:15}
\end{align}
A product of two Wigner matrices is given in terms of the Clebsch--Gordan coefficients $C^{JM}_{\ell_{1}m_{1};\ell_{2}m_{2}}$ by
\begin{align}
 \mathcal{D}^{\ell_{1}}_{m_{1}n_{1}}(R)\mathcal{D}^{\ell_{2}}_{m_{2}n_{2}}(R)=\sum_{J=|\ell_{1}-\ell_{2}|}^{\ell_{1}+\ell_{2}}\sum_{M,N=-J}^{J}C^{JM}_{\ell_{1}m_{1};\ell_{2}m_{2}}C^{JN}_{\ell_{1}n_{1};\ell_{2}n_{2}}\mathcal{D}^{J}_{MN}(R)\,.\label{eq:14}
\end{align}

We will now use these decompositions to write the convolutions~\eqref{eq:28} and \eqref{SO3C_conv} in the Fourier domain. To this end, we use Greek letters to index vectors in the spaces $V_{1}$ and $V_{2}$ in which the feature maps take values.
\begin{proposition}
  The Fourier transform of the spherical convolution~\eqref{eq:28} with $\mathcal{X}=S^{2}$ and $\mathcal{Y}=\SO(3)$ is given by
\begin{align}
  [\widehat{(\kappa \star f)_{\mu}}]^{\ell}_{mn} &= \sum_{\nu=1}^{\dim V_{2}}\sum_{\sigma,\tau=1}^{\dim V_{1}}\sum_{\substack{\ell_{i}=0\\i=1,2,3}}^{\infty}\sum_{\substack{m_{i},n_{i}=-\ell_{i}\\i=1,2,3}}^{\ell_{i}}\sum_{J=|\ell_{2}-\ell_{1}|}^{\ell_{2}+\ell_{1}}\sum_{M,N=-J}^{J}C^{JM}_{\ell_{2}m_{2};\ell_{1}n_{1}}C^{JN}_{\ell_{2}n_{2};\ell_{1}m_{1}}\nonumber\\
  &\qquad C^{\ell m}_{JM;\ell_{3}m_{3}}C^{\ell n}_{JN;\ell_{3}n_{3}}\widehat{(\rho_{2,\mu\nu})}^{\ell_{2}}_{m_{2}n_{2}}\widehat{(\kappa_{\nu\sigma})}^{\ell_{1}}_{m_{1}}\overline{\widehat{\rho_{1,\sigma\tau}}^{\ell_{3}}_{n_{3}m_{3}}}\overline{\widehat{(f_{\tau})}^{\ell_{1}}_{n_{1}}}\,.\label{eq:9}
\end{align}
\end{proposition}
For $\rho_{1}=\rho_{2}=\mathrm{id}$, \eqref{eq:9} simplifies to
\begin{align}
  [\widehat{(\kappa \star f)}_{\mu}]^{\ell}_{mn} = \sum_{\nu=1}^{\dim V_{1}} (\widehat\kappa_{\mu\nu})^{\ell}_{n}\overline{(\widehat{f_{\nu}})^{\ell}_{m}} \,.\label{eq:12}
\end{align}
A similar calculation can be performed for input features in $\SO(3)$ as detailed by the following proposition.
\begin{proposition}
The Fourier transform of the spherical convolution~\eqref{SO3C_conv} with $\mathcal{X}=\mathcal{Y}=\SO(3)$ can be written in the Fourier domain as
\begin{align}
  [\widehat{(\kappa \star f)}]^{\ell}_{mn} &=\frac{8\pi^{2}}{2\ell+1}\sum_{p=-\ell}^{\ell}\sum_{\substack{\ell_{i}=0\\i=1,2,3}}^{\infty}\sum_{\substack{m_{i},n_{i}=-\ell_{i}\\i=1,2,3}}^{\ell_{i}}\sum_{J=|\ell_{1}-\ell_{2}|}^{\ell_{1}+\ell_{2}}\sum_{M,N=-J}^{J}C^{JM}_{\ell_{1}m_{1};\ell_{2}m_{2}}C^{JN}_{\ell_{1}n_{1};\ell_{2}n_{2}}\nonumber\\
  &\qquad C^{\ell m}_{JM;\ell_{3}m_{3}}C^{\ell p}_{JN;\ell_{3}n_{3}}\widehat{\rho_{2}}^{\ell_{1}}_{m_{1}n_{1}}\cdot\widehat{\kappa}^{\ell}_{pn}\cdot\overline{\widehat{\rho_{1}}^{\ell_{2}}_{n_{2}m_{2}}}\cdot\widehat{f}^{\ell_{3}}_{m_{3}n_{3}}\,.\label{eq:6}
\end{align}
Here, the dot $\cdot$ denotes matrix multiplication in $V_{1,2}$, as spelled out in~\eqref{eq:9}.
\end{proposition}
For $\rho_{1}=\rho_{2}=\id$ \eqref{eq:6} becomes
\begin{align}
  [\widehat{(\kappa \star f)}]^{\ell}_{mn} &=\frac{8\pi^{2}}{2\ell+1}\sum_{p=-\ell}^{\ell}\widehat{\kappa}^{\ell}_{pn}\cdot\widehat{f}^{\ell}_{mp}\,.
\end{align}
Note that in all these expressions, the Fourier transform is done component wise with respect to the indices in $V_{1,2}$.

\subsection{Decomposition into irreducible representations}
\label{sec:decomp-into-irreps}
An immediate simplification of~\eqref{eq:9} and \eqref{eq:6} can be achieved by decomposing $\rho_{1,2}$ into irreps of $\SO(3)$ which are given by the Wigner matrices $\mathcal{D}^{L}$,
\begin{align}
  \rho(R) = \bigoplus_{\lambda}\bigoplus_{\mu}\mathcal{D}^{\lambda}(R)\,,\label{eq:34}
\end{align}
where $\mu$ counts the multiplicity of $\mathcal{D}^{\lambda}$ in $\rho$. Correspondingly, the spaces $V_{1,2}$ are decomposed according to $V_{1,2}=\bigoplus_{\lambda}\bigoplus_{\mu} V_{1,2}^{\lambda\mu}$, where $V_{1,2}^{\lambda\mu}=\RR^{2\lambda+1}$. The feature maps then carry indices $f^{\lambda\mu}_{\nu}$ with $\lambda=0,\dots,\infty$, $\mu=1,\dots,\infty$, $\nu=-\lambda,\dots,\lambda$ with only finitely many non-zero components. Using this decomposition of $V_{1,2}$ the convolution~\eqref{eq:28} is given by
\begin{align}
  (\kappa\star f)^{\lambda\mu}_{\nu}(R) = \sum_{\rho=-\lambda}^{\lambda}\sum_{\theta=0}^{\infty}\sum_{\sigma=1}^{\infty}\sum_{\tau,\pi=-\theta}^{\theta}\int_{S^{2}}\mathcal{D}^{\lambda}_{\nu\rho}(R)\kappa^{\lambda\mu;\theta\sigma}_{\rho;\tau}(R^{-1}x)\mathcal{D}^{\theta}_{\tau\pi}(R^{-1})f^{\theta\sigma}_{\pi}(x)\dd{x}\,.
\end{align}
By plugging these expressions for $\rho_{1,2}$, $\kappa$ and $f$ into~\eqref{eq:9}, we obtain the following proposition.
\begin{proposition}\label{prop:decomp_s2_conv}
  The decomposition of~\eqref{eq:9} into representation spaces of irreducible representations of $\SO(3)$ is given by
\begin{align}
  [\widehat{(\kappa \star f)^{\lambda\mu}_{\nu}}]^{\ell}_{mn} &=\sum_{\rho=-\lambda}^{\lambda}\sum_{\theta=0}^{\infty}\sum_{\sigma=1}^{\infty}\sum_{\tau,\pi=-\theta}^{\theta} \sum_{j=0}^{\infty}\sum_{q,r=-j}^{\ell_{i}}\sum_{J=|\ell_{2}-j|}^{\ell_{2}+j}\sum_{M,N=-J}^{J}C^{JM}_{\lambda\nu;jr}C^{JN}_{\lambda\rho;jq}\nonumber\\
  &\qquad C^{\ell m}_{JM;\theta\tau}C^{\ell n}_{JN;\theta\pi}(\widehat{\kappa^{\lambda\mu;\theta\sigma}_{\rho;\tau}})^{j}_{q} \overline{(\widehat{f^{\theta\sigma}_{\pi}})^{j}_{r}}\,.
\end{align}
Similarly, \eqref{eq:6} decomposes according to
\begin{align}
  (\widehat{(\kappa\star f)^{\lambda\mu}_{\nu}})^{\ell}_{mn}&=\frac{8\pi^{2}}{2\ell+1}\sum_{\rho=-\lambda}^{\lambda}\sum_{\theta=0}^{\infty}\sum_{\sigma=1}^{\infty}\sum_{\tau,\pi=-\theta}^{\theta}\sum_{p=-\ell}^{\ell}\sum_{j=0}^{\infty}\sum_{q,r=-j}^{j}\sum_{J=|\lambda-\sigma|}^{\lambda+\sigma}\sum_{M,N=-J}^{J}C^{JM}_{\lambda\nu;\theta\tau}C^{JN}_{\lambda\rho;\theta\pi}\nonumber\\
  &\qquad C^{\ell m}_{JM;jq}C^{\ell p}_{JN;jr}(\widehat{\kappa^{\lambda\mu;\theta\sigma}_{\rho;\tau}})^{\ell}_{pn}(\widehat{f^{\theta\sigma}_{\pi}})^{j}_{qr}\,.\label{eq:29}
\end{align}
\end{proposition}
In these expressions, the Fourier transform of the convolution is given entirely in terms of the Fourier transforms of the kernel and the input feature map, as well as Clebsch--Gordan coefficients. In particular, Fourier transforms of the representation matrices $\rho_{1,2}$ are trivial in this decomposition of the spaces $V_{1}$ and $V_{2}$.

\subsection{Output features in $\SE(3)$}\label{ex:SE3Outputs}
  As an example of a possible application of the techniques presented in this section, consider the problem of 3D object detection in pictures taken by fisheye cameras. These cameras have a spherical image plane and therefore, the components of the input feature map $f$ transform as scalars under the regular representation (cf.~\eqref{eq:2}):
\begin{align}
  [\pi_{1}(R)f](x)=f(R^{-1}x)\,.
\end{align}
Since this is the transformation property considered in the context of spherical CNNs, the entire network can be built using the layers discussed in this section.
  
  As detailed in Section~\ref{sec:obj_detection}, for object detection, we want to identify the class, physical size, position and orientation for each object in the image. This can be realized by associating to each pixel in the output picture (which is often of lower resolution than the input) a class probability vector $p\in P(\Omega)$, a size vector $s\in\RR^{3}$ containing height, width and depth of the object, a position vector $x\in\RR^{3}$ and an orientation given by a matrix $Q\in\SO(3)$. Here, $P(\Omega)$ is the space of probability distributions in $\Nc$ classes as in~\eqref{eq:35}. In the framework outlined above, this means that the output feature map takes values in $P(\Omega)\oplus\RR^{3}\oplus\RR^{3}\oplus\SO(3)$.

  If the fisheye camera rotates by $R\in\SO(3)$, the output features have to transform accordingly. In particular, since the classification and the size of the object do not depend on the rotation, $p$ transforms as $\Nc$ scalars and $s$ transforms as three scalars:
\begin{align}
  \rho_{2}(R) p = p, \qquad \rho_{2}(R) s = s\,,\label{eq:30}
\end{align}
where we used the notation introduced in~\eqref{eq:3}. The position vector $x$ on the other hand transforms in the fundamental representation of $\SO(3)$
\begin{align}
  \rho_{2}(R)x = R\cdot x\,.\label{eq:31}
\end{align}
Finally, the rotation matrix $Q$ transforms by a similarity transformation
\begin{align}
  \rho_{2}(R)Q = R\cdot Q \cdot R^{T}\,.\label{eq:32}
\end{align}

As described above for the general case, the transformation property~\eqref{eq:30}--\eqref{eq:32} of the output feature map can be decomposed into a direct sum of irreducible representations, labeled by an integer $\ell$. The scalar transformations of~\eqref{eq:30} are $\Nc+3$ copies of the $\ell=0$ representation and the fundamental representation in~\eqref{eq:31} is the $\ell=1$ representation. To decompose the similarity transformation in~\eqref{eq:32}, we use the following
\begin{proposition}
Let $A$, $B$, $C$ be arbitrary matrices and $\vrize(M)$ denote the concatenation of the rows of the matrix $M$. Then,
  \begin{align}
  \vrize(A\cdot B\cdot C)=(A\otimes C^{T})\cdot\vrize(B)\,.\label{eq:33}
\end{align}
\end{proposition}
With this, we obtain for~\eqref{eq:32}
\begin{align}
  \rho_{2}(R)\vrize(Q) = (R\otimes R)\cdot \vrize(Q)\,,
\end{align}
i.e.\ $Q$ transforms with the tensor product of two fundamental representations. According to~\eqref{eq:14}, this tensor product decomposes into a direct sum of one $\ell=0$, one $\ell=1$ and one $\ell=2$ representation. In total, the final layer of the network will therefore have (in the notation introduced below~\eqref{eq:34}) $\lambda=0,1,2$, $\nu=-\lambda,\dots,\lambda$ and $\mu=1,\dots, \Nc+4$ for $\lambda=0$, $\mu=1,2$ for $\lambda=1$ and $\mu=1$ for $\lambda=2$.

Note that the transformation properties~\eqref{eq:30}--\eqref{eq:32} of the output feature map are independent of the transformation properties of the input feature map. We have restricted the discussion here to fisheye cameras since, as stated above, these can be realized by the spherical convolutions considered in this section. For pinhole cameras on the other hand, the representation $\pi_{1}$ acting on the input features will be a complicated non-linear transformation arising from the projection of the transformation in 3D space onto the flat image plane. Working out the details of this representation is an interesting direction for further research.
  


\subsection{$\SE(3)$ equivariant networks}
The same decomposition of $V_{1,2}$ into representation spaces of irreducible representations of $\SO(3)$, which was used in Section~\ref{sec:decomp-into-irreps} can also be used to solve the kernel constraint~\eqref{eq:10} for equivariant networks of $\SE(3)$, as discussed in \cite{weiler2018}. In this section, we review this construction.

In the decomposition into irreps, the kernel constraint~\eqref{eq:10} reads
\begin{align}
  \kappa^{\lambda\mu;\theta\sigma}_{\rho;\tau}(Ry)=\sum_{\nu=-\lambda}^{\lambda}\sum_{\pi=-\theta}^{\theta}\mathcal{D}^{\lambda}_{\rho\nu}(R)\,\kappa^{\lambda\mu;\theta\sigma}_{\nu;\pi}(y)\,\mathcal{D}^{\theta}_{\pi\tau}(R^{-1})\,.\label{eq:11}
\end{align}
In the following, we will use $\cdot$ to denote matrix multiplication in $\rho,\nu,\pi,\tau$ and drop the multiplicity indices $\mu,\sigma$ since~\eqref{eq:11} is a component-wise equation with respect to the multiplicity.

On the right-hand side of~\eqref{eq:11}, $\SO(3)$ acts in a tensor product representation on the kernel. To make this explicit, we use the vectorization~\eqref{eq:33} and  the unitarity of the Wigner matrices to rewrite~\eqref{eq:11} into\footnote{Note that there is a typo in the corresponding equation (13) in \cite{weiler2018}, where the complex conjugation is missing.}
\begin{align}
  \vrize(\kappa^{\lambda\theta}(Ry)) = (\mathcal{D}^{\lambda}(R)\otimes \overline{\mathcal{D}^{\theta}}(R))\cdot\vrize(\kappa^{\lambda\theta}(y))\,.
\end{align}
Using~\eqref{eq:13} and \eqref{eq:14}, we can decompose the tensor product of the two Wigner matrices into a direct sum of Wigner matrices $\mathcal{D}^{J}$ with $J=|\lambda-\theta|,\dots,\lambda+\theta$. Performing the corresponding change of basis for $\vrize(\kappa^{\lambda\theta})$ leads to components $\vrize(\kappa^{\lambda\theta;J})$ on which the constraint takes the form
\begin{align}
  \vrize(\kappa^{\lambda\theta;J}(Ry))=\mathcal{D}^{J}(R)\cdot\vrize(\kappa^{\lambda\theta;J}(y))\,.\label{eq:17}
\end{align}
According to~\eqref{eq:16} and \eqref{eq:15}, the spherical harmonics $Y^{\ell}_{m}$ solve this constraint and they in fact span the space of solutions with respect to the angular dependence of $\kappa^{\lambda\theta,J}$. Therefore, a general solution of~\eqref{eq:17} has the form
\begin{align}
  \vrize(\kappa^{\lambda\theta;J}(y))=\sum_{k}\sum_{m=-J}^{J}w^{\lambda\theta;J}_{k,m}\varphi^{k}(||y||)Y^{J}_{m}(y)\,,
\end{align}
with radial basis functions $\varphi^{k}$ and (trainable) coefficients $w$.

As an example of an application of group equivariant network architectures, we considered spherical CNNs in this section, which are of great practical importance. Spherical convolutions serve as a good example of the Fourier perspective on group equivariant convolutions since the spectral theory on the sphere and rotation group $\SO(3)$ is well-understood. Consequently, in Proposition~\ref{prop:decomp_s2_conv}, we could give explicit, yet completely general expressions for spherical convolutions for feature maps transforming in arbitrary representations of $\SO(3)$, given just in terms of Clebsch--Gordan coefficients.

In principle, such expressions could be derived for a large class of symmetry groups. The foundation of this generalization was laid in~\cite{lang2020}, where it was shown how the kernel constraint for any compact symmetry group can be solved in terms of well-known representation theoretic quantities. In position space, algorithms already exist which can solve the symmetry constraint and generate equivariant architectures automatically~\cite{finzi2021}. 
